A Unified Speech LLM for Diarization and Speech Recognition in Multilingual Conversations

Speech Large Language Models (Speech LLMs) have emerged as a crucial paradigm in recent years, extending the capabilities of traditional LLMs to speech tasks such as automatic speech recognition (ASR) and spoken dialogue modeling. However, their effectiveness in real-world multilingual conversations remains limited by the scarcity of data that captures natural conversational phenomena. To address this, the MLC-SLM Challenge provides a multilingual conversational dataset and evaluates models on two tasks: ASR with oracle segmentation (Task I) and joint diarization and recognition without oracle information (Task II). In this paper, we focus on Task II and propose a unified speech LLM that jointly performs diarization and ASR in an end-to-end manner. By reformulating the training data format and modifying the inference procedure, our model addresses the ambiguity inherent in pre-segmented audio and achieves a 54.87\% relative improvement in tcpWER/tcpCER over the baseline, ranking 8th overall, despite using a smaller LLM backbone. We also report results from Task I using a fine-tuned speech LLM.

==> experiment.tex <==
\subsection{Datasets}

\textbf{Training set}
The training set (Train) comprises approximately 11 languages: English (en), French (fr), German (de), Italian (it), Portuguese (pt), Spanish (es), Japanese (jp), Korean (ko), Russian (ru), Thai (th), Vietnamese (vi).

Each recording consists of two-speaker conversational speech on randomly assigned topics.

Conversations are natural and fluent, with speakers engaging in meaningful dialogues on each topic.

Recorded in quiet indoor environments using devices such as iPhones.

Each recording will provide the oracle segmentation and speaker label for the development of speech recognition and speaker diarization systems.

Both Task I and Task II share the same training set.

The English dataset comprises approximately 500 hours of recordings from various regions, including British, American, Australian, Indian, and Philippine English. Other languages contribute around 100 hours each, resulting in a total of approximately 1500 hours of multilingual conversational speech data.

This dataset is designed to provide a rich resource for training and evaluating multilingual conversational speech language models (MLC-SLM), addressing the challenges of linguistic diversity, speaker variability, and contextual understanding.

\textbf{Development set} The development set (Dev) has the same setting as the training set but contains approximately 4 hours of recordings for each language. Both Task I and Task II share the same development set.

\textbf{Evaluation set} Different evaluation sets are employed for each task, designated as Eval\_1 and Eval\_2. Specifically, Eval\_1 includes oracle timestamps and speaker labels, which are evaluated using WER/CER. Eval\_2 does not provide timestamps or speaker labels, necessitating a speaker diarization (SD) system to segment the longer recordings before recognition.
Participants can access the dataset by signing the Data use agreement and submitting to the registration form. After submission, the data download link will be sent to your email.
